LiteTransformerSearch: Training-free Neural Architecture Search for Efficient Language Models

The Transformer architecture is ubiquitously used as the building block of large-scale autoregressive language models. However, finding architectures with the optimal trade-off between task performance (perplexity) and hardware constraints like peak memory utilization and latency is non-trivial. This is exacerbated by the proliferation of various hardware. We leverage the somewhat surprising empirical observation that the number of decoder parameters in autoregressive Transformers has a high rank correlation with task performance, irrespective of the architecture topology. This observation organically induces a simple Neural Architecture Search (NAS) algorithm that uses decoder parameters as a proxy for perplexity without need for any model training. The search phase of our training-free algorithm, dubbed Lightweight Transformer Search (LTS), can be run directly on target devices since it does not require GPUs. Using on-target-device measurements, LTS extracts the Pareto-frontier of perplexity versus any hardware performance cost. We evaluate LTS on diverse devices from ARM CPUs to NVIDIA GPUs and two popular autoregressive Transformer backbones: GPT-2 and Transformer-XL. Results show that the perplexity of 16-layer GPT-2 and Transformer-XL can be achieved with up to 1.5x, 2.5x faster runtime and 1.2x, 2.0x lower peak memory utilization. When evaluated in zero and one-shot settings, LTS Pareto-frontier models achieve higher average accuracy compared to the 350M parameter OPT across 14 tasks, with up to 1.6x lower latency. LTS extracts the Pareto-frontier in under 3 hours while running on a commodity laptop. We effectively remove the carbon footprint of hundreds of GPU hours of training during search, offering a strong simple baseline for future NAS methods in autoregressive language modeling.

==> LTS_Version2 2/1_intro.tex <==
\vspace{-0.1cm}
\section{Introduction}\label{sec:intro}
\vspace{-0.1cm}
The Transformer architecture~\citep{vaswani2017attention} has been used as the de-facto building block of most pre-trained language models like GPT~\citep{brown2020language}. A common problem arises when one tries 
to create smaller versions of Transformer models for edge or real-time applications (e.g. text prediction) with strict memory and latency constraints: it is not clear
what the architectural hyperparameters should be, e.g., number of attention heads, number of layers, embedding dimension, and the inner dimension of the feed forward network, etc. This problem is exacerbated if each
Transformer layer is allowed the freedom to have different values for these settings. 
This results in a combinatorial explosion of architectural hyperparameter choices and a large heterogeneous search space. For instance, the
search space considered in this paper consists of over $10^{54}$ possible architectures.

Neural Architecture Search (NAS) is an organic solution due to its ability to automatically search
through candidate models with multiple conflicting objectives like latency vs. task performance.
The central challenge in NAS is the prohibitively expensive function evaluation, i.e., evaluating each architecture requires training it on the dataset at hand. Thus it is often infeasible to evaluate more than a handful of architectures during the search phase. 
% NAS has made tremendous advances recently where search can often proceed in less than one GPU day on a single workstation~\cite{} as opposed to early attempts~\cite{} which required thousands of GPU hours. 
Supernets~\cite{pham2018efficient} have emerged as a dominant 
paradigm in NAS which combine all 
possible architectures into a single graph and jointly train them using weight-sharing. 
% This also is usually termed as one-shot methods. 
Nevertheless, supernet training imposes constraints
on the expressiveness of the search space~\cite{ning2021evaluating} and is often memory-hungry~\cite{pcdarts,ofa,analyzingnas}
as it creates large networks during search. Additionally, training supernets is non-trivial as children architectures may interfere with each other and the ranking between sub-architectures based on task performance is not preserved~\cite{ning2021evaluating}\footnote{See \citep{ning2021evaluating} for a comprehensive treatment of the difficulties of training supernets.}. 

We consider a different approach by proposing a training-free proxy that provides a highly accurate ranking of candidate architectures during NAS without need for costly function evaluation or supernets. Our scope is NAS for efficient autoregressive Transformers used in language modeling. We design a lightweight search method that is target hardware-aware and outputs a gallery of 
models on the Pareto-frontier of perplexity versus hardware metrics. We term this method Lightweight Transformer Search (\sys{}). \sys{} relies on our somewhat surprising observation: {\textit{the decoder parameter count
has a high rank correlation with the perplexity of fully trained autoregressive Transformers.}} 

Given a set of autoregressive Transformers, one can accurately rank them using decoder parameter count as the proxy for perplexity. Our observations are also well-aligned with the power laws in~\cite{kaplan2020scaling}, shown for homogeneous autoregressive Transformers, i.e., when all decoder layers have the same configuration. We provide extensive experiments that establish a high rank correlation between perplexity and decoder parameter count for \emph{both} homogeneous and heterogeneous search spaces. 
% on popularly used autoregressive Transformer backbone.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/overview.pdf}
%     % \vspace{-0.5cm}
%     \caption{High-level overview of \sys{}. We propose a zero-cost proxy for evaluating the validation perplexity of candidate architecture candidates. Our search is powered by evolutionary algorithms which use the proposed proxy along with real latency measurements on the target hardware to evaluate sampled architectures.}
%     \label{fig:overview}
% % \vspace{-0.5cm}
% \end{figure}

\begin{SCfigure}[50][t]
    \centering
    \includegraphics[width=0.45\columnwidth]{figures/overview.pdf}
    % \vspace{-0.5cm}
    \caption{High-level overview of \sys{}. We propose a training-free zero-cost proxy for evaluating the validation perplexity of candidate architectures. Pareto-frontier search is powered by evolutionary algorithms which use the proposed proxy along with real latency and memory measurements on the target hardware to evaluate sampled architectures.}
    \label{fig:overview}
\vspace{-0.5cm}
\end{SCfigure}

The above phenomenon coupled with the fact that a candidate architecture's hardware performance can be measured on the target device 
% \footnote{An insight noted in \cite{elsken2018lemonade} and \cite{guerrero2021bagofbaselines} that we leverage during search.}
% by passing through a single minibatch (often batch size $1$ for inference)
leads to a training-free search procedure: {\textit{pick one's favorite discrete search algorithm 
(e.g. evolutionary search), sample candidate architectures from the search space; count their decoder parameters as a proxy for task performance (i.e., perplexity); measure their hardware performance (e.g., latency and memory) directly on the target device; and progressively create a Pareto-frontier estimate.}} While we have chosen a reasonable search algorithm in this work, one can plug and play any Pareto-frontier search method such as those in \cite{guerrero2021bagofbaselines}.

Building upon these insights, Figure~\ref{fig:overview} shows a high-level overview of \sys{}. We design the first training-free Transformer search that is performed entirely on the target (constrained) platform. 
% We design the first on-target-device Transformer search that eliminates the need for high-end GPUs, enabling direct search on the (edge) target platform. 
As such, \sys{} easily performs a multi-objective NAS where several underlying hardware performance metrics, e.g., latency and peak memory utilization, are simultaneously optimized. Using our training-free proxy, we extract the $3$-dimensional Pareto-frontier of perplexity versus latency and memory in a record-breaking time of $<3$ hours on a commodity Intel Core i7 CPU. Notably, \sys{} eliminates the carbon footprint from hundreds of GPU hours of training associated with legacy NAS methods. 

\comment{
Once the Pareto-frontier models are identified, the user can pick a model based on their desired hardware constraints and fully train it on the target dataset. We note that the cost of training this model is lower than the cost of training large supernets, particularly since our NAS is focused on low-latency and memory-efficient Transformers. \sys{} also avoids the many difficulties associated with training supernets
% like gradient interference between subgraphs, large memory footprint and the inability to have an expressive search space as the subgraphs must strictly fit in the supergraph for weight-sharing to be efficient. 
\footnote{See \citep{ning2021evaluating} for a comprehensive treatment of the difficulties of training supernets.}.
}

To corroborate the effectiveness of our proxy, we train over $2900$ Transformers on three large language modeling benchmark datasets, namely, WikiText-103~\cite{merity2016pointer}, One Billion Word~\cite{chelba2013one}, and Pile~\cite{gao2020pile}. We use \sys{} to search for Pareto-optimal architectural hyperparameters in two popularly used autoregressive Transformer backbones, namely, Transformer-XL~\cite{dai2019transformer} and GPT-2~\cite{radford2019language}. We believe decoder parameter count should be regarded as a competitive baseline for evaluating Transformer NAS, both in terms of ranking capabilities and easy computation. We open-source our code along with tabular information of our trained models to foster future NAS research on Transformers.

% \mojan{add OPT results in the abtrsact and intro}

% In summary the contributions of this paper are as follows:
% \begin{itemize}
%     \item Proposing decoder parameter count as a zero-cost proxy for ranking Transformer architectures during NAS. 
    % \item Repurposing CNN architecture ranking proxies~\cite{abdelfattah2020zero} for Transformer architectures and evaluating their performance compared to decoder parameter count.
    % \item Designing the first on (edge) target-device NAS pipeline which eliminates the need for high-end GPUs to conduct NAS, thereby enabling direct search on the target commodity platform. Using our training-free proxy, we can extract the perplexity versus latency Pareto-frontier of Transformers in a record breaking time of $<3$ hours on a commodity Intel Core i7 CPU.
    % \item Providing large-scale proof-of-concept experiments on the effectiveness of our training-free proxies for two language datasets and a wide range of model sizes.
% \end{itemize}

% \input{1_0_intro_old}



==> LTS_Version2 2/2_related_work.tex <==
\vspace{-0.2cm}
\section{Related Work}\label{sec:related_work}
\vspace{-0.2cm}
Here, we discuss literature on automated search for Transformer architectures in the language domain. We refer to extensive surveys on NAS~\citep{elsken2019neural,wistuba2019survey} for a broader overview
of the field. 

\noindent \textbf{Decoder-only Architectures.} \citet{primer} search over TensorFlow programs that implement an autoregressive language model via evolutionary search. 
% use evolutionary search on a large search space where the Transformer layers can be composed of primitive TensorFlow operation sequences.
% This is essentially searching over possible TensorFlow programs that implement an autoregressive language model via evolutionary search. 
Since most random sequences of programs either
have errors or underperform, the search has to be seeded with the 
regular Transformer architecture, termed ``Primer''. As opposed to ``Primer'' which 
uses large computation to search a general space, we aim 
to efficiently search the ``backbone'' of traditional 
decoder-only Transformers. Additionally, the objective in ``Primer'' is to find models that train faster. Our objective for NAS, however, is to deliver Pareto-frontiers for inference, with respect to perplexity and hardware constraints. 

\noindent \textbf{Encoder-only Architectures.} Relative to decoder-only 
autoregressive language models, encoder-only architectures
like BERT~\cite{devlin2019bert} have received much more recent attention from the NAS community. NAS-BERT~\cite{nasbert} trains a supernet to efficiently search for
masked language models (MLMs) which are compressed versions of the standard BERT,
% in a task-agnostic manner. 
Such models can then be used in downstream 
tasks as is standard practice. 
Similar to NAS-BERT,~\citet{analyzingnas} train 
a supernet to conduct architecture 
search with the aim of finding more efficient BERT variants. They find interesting 
empirical insights into supernet training issues like differing gradients at the same 
node from different child architectures and different tensors as input and output 
at every node in the supernet. The authors propose fixes
that significantly improve supernet training. \citet{fasttransformers,autotinybert,autobertzero}
also conduct variants of supernet training with the aim of finding
more efficient BERT models.

% \cite{bort} pose the problem of optimizing for inference speed, 
% parameter size, and task accuracy as an approximate optimization problem that can 
% be solved efficiently for architectures that are mainly determined by the number of 
% encoder parameters for inference speed and number of parameters. Since BERT-style 
% search spaces (number of encoder layers, number of attention heads, hidden size and 
% intermediate layer size) \dey{we need to put the search space description 
% in the same terminology as the rest of the paper.} satisfy these constraints they 
% apply approximate optimization to extract efficient sub-architectures.

% Finding Fast Transformers: One-shot NAS by Component Composition 2020:
% Similar to NAS-BERT and Analyzing, \cite{fasttransformers} search for faster BERT-base 
% models. They take the approach of decomposing the transformer architecture into
% smaller components and use a sampling-based search method to find optimal 
% models for inference.

% Autotinybert: Automatic Hyperparameter optimization for language models 2021:
% Similar to NAS-BERT and Analyzing and Fast Transformers, \cite{autotinybert} they conduct a 
% supernet based search on the BERT search space for searching efficient 
% models with lower latency.

% AutoBertZero: Evolving the backbone from scratch 2021:
% \cite{autobertzero} et al. construct a novel search space for BERT-like models. 
% Specifically they intersperse a searched convolution layer amongst 
% attention layers. Attention layers are also searched from
% sequences of primitive mathematical operations. Search is carried 
% out via evolutionary methods but since candidate evaluations 
% on such a large search space will be prohibitive they first train
% a supernet. Then child architectures sampled via evolutionary search
% inherit weights from the corresponding parts of the supernet and are 
% then finetuned for a small number of steps.

\noindent \textbf{Encoder-Decoder Related:} Applying the well-known DARTS~\cite{liu2018darts} approach to 
Transformer search spaces leads to memory-hungry supernets. To mitigate this issue, \citet{memoryefficientsearch} propose a multi-split reversible network and a memory-efficient
backpropagation algorithm. One of the earliest papers 
that applied discrete NAS to Transformer search spaces
was \cite{evolvedtransformer}, which uses a modified form of evolutionary search. 
Due to the expense of directly performing discrete search on the search space, 
this work incurs extremely large computation overhead.
Follow-up work by~\cite{wang2020hat} uses the Once-For-All~\cite{ofa} approach to train a supernet for encoder-decoder architectures used in machine translation. Search is performed on subsamples of the supernet that inherit weights to estimate task accuracy. For each target device, the authors train a small neural network regressor on thousands of architectures to estimate latency.
% build a 'simulator' by sampling thousands of smaller architectures from the supernet and measuring their latencies.
% This data is then used to train a small neural network regressor which predicts the latency of input architectures.
% Since this latency estimator is cheap to,  evolutionary algorithms can be used to conduct the search. 
As opposed to using a latency estimator, \sys{} evaluates the latency of each candidate architecture on the target hardware. Notably, by performing the search directly on the target platform, \sys{} can easily incorporate various hardware performance metrics, e.g., peak memory utilization, for which accurate estimators may not exist. To the best of our knowledge, such holistic integration of multiple hardware metrics in Transformer NAS has not been explored previously.
% \mojan{mention how we contrast from them since we measure not simulate the latency: As opposed to using a latency estimator, we directly evaluate the latency of each model on the target device.}


% \textbf{Vision tasks related}

% Vision Transformer Architecture Search

% UniNet

% Searching the search space of Vision Transformer

% Searching for Efficient Multi-Stage Vision Transformers

% GLiT: NAS for global and local image transformer

% BossNAS: Exploring Hybrid CNN-transformers with Block-wisely Self-supervised NAS

% Autoformer: Searching transformers for vision

% Auto Learning Attention via NAS 2020









==> LTS_Version2 2/3_2_1_pruning.tex <==
% \subsubsection{Low-cost Ranking Proxies}\label{sec:pruning}
\noindent\textbf{$\blacktriangleright$ Low-cost Ranking Proxies.}
Recently, \citet{abdelfattah2020zero} utilize the summation of pruning scores over all model
weights as the ranking proxy for Convolutional Neural Networks (CNNs), where a higher score corresponds to higher architecture rank in the search space. \citet{colin2022adeeperlook} analyze these and more recent proxies and find that no particular proxy performs consistently well over various tasks and baselines, while parameter and floating point operations (FLOPS) count proxies are quite competitive. However, they did not include Transformer-based search spaces in their analysis. 
To the best of our knowledge, low-cost (pruning-based) proxies have not been evaluated on Transformer search spaces in the  language domain. Note that one cannot naively apply these proxies to language models. Specifically, since the embedding layer in Transformers is equivalent to a lookup operation, special care must be taken to omit this layer from the proxy computation. Using this insight, we perform the first systematic study of low-cost proxies for NAS on autoregressive Transformers for text prediction. 
% To evaluate candidate architectures, we calculate the accumulated pruning score assigned to model parameters. 

We leverage various pruning metrics, namely, \gradnorm, \snip~\cite{lee2018snip}, \grasp~\cite{wang2020picking}, \fisher~\cite{theis2018faster}, and \synflow~\cite{tanaka2020pruning}. We also study \jacobcov~\cite{mellor2020neural} and
\relulogdet~\cite{mellor2021neural} which are low-cost scoring mechanisms proposed for NAS on CNNs in vision tasks. 
While these low-cost techniques do not perform model training, they require forward and backward passes over the architecture to compute the proxy, which can be time-consuming on low-end hardware. Additionally, the aforesaid pruning techniques, by definition, incorporate the final softmax projection layer in their score assessment. Such an approach seems reasonable for CNNs dealing with a few classification labels, however, it can skew the evaluation for autoregressive Transformers dealing with a large output vocabulary space. 
To overcome these shortcomings, we introduce a zero-cost architecture ranking strategy in the next section that outperforms the proposed low-cost proxies in terms of ranking precision, is data free, and does not perform any forward/backward propagation.

% The synaptic flow introduced in~\cite{tanaka2020pruning} assigns an importance score to \edit{CNN} weights that can be used to prune redundant parameters without need for training or utilizing data. Followup work~\cite{abdelfattah2020zero} has utilized the summation of synaptic flow score over all model weights to perform zero-shot NAS on CNNs. We adapt the formulation of synaptic flow to Transformer architectures. Specifically, since the embedding layer in Transformer architectures is equivalent to a look up table, we remove this layer in our analysis of the synaptic flow. 

% As shown in Figure~\ref{fig:proxies}, the synaptic flow proxy performs on par with partial training in terms of architecture ranking capabilities while incurring zero training cost. Therefore, the synaptic flow proxy improves the runtime for NAS by an average of \edit{$XXX$}. \edit{While synaptic flow does not require model training, it still requires one forward and backward pass over the architecture to compute the parameter scores, which can be time consuming on commodity hardware. Recent work~\cite{} has shown that the synaptic flow measure is equivalent to a soft parameter counter. As such, we propose to utilize the number of model parameters as a proxy for validation perplexity.} 


==> LTS_Version2 2/3_2_2_decoder_params.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/params_corr_all.png}
    \vspace{-0.2cm}
    \caption{Our training-free zero-cost proxy based on decoder parameter count is highly correlated with the (ground truth) validation perplexity after full training. Each plot contains $200$ architectures sampled randomly from the search space of Transformer-XL or GPT-2 backbone.}\label{fig:zero_proxy}
% experiments: mem_transformer (fear_stage_1_heterogeneous, lm1b_random), GPT2 (random_hf_gpt2_flex_wt103_random_d_embed, random_hf_gpt2_flex_lm1b)
\vspace{-0.6cm}
\end{figure}

% \vspace{-0.2cm}
% \subsubsection{Decoder Parameter Count as a Proxy}\label{sec:param_proxy}
\noindent\textbf{$\blacktriangleright$ Decoder Parameter Count as a Proxy.} We empirically establish a strong correlation between the parameter count of decoder layers and final model performance in terms of validation perplexity. 
% \edit{Our findings are also well-aligned with the scaling laws introduced in~\cite{kaplan2020scaling} which show a power-law relationship between model size and crossentropy loss.} 
% We thus propose utilizing the decoder parameter count as a zero-cost proxy for relative ranking of architectures during NAS. 
We evaluate $200$ architectures sampled uniformly at random from the search space of two autoregressive Transformer backbones, namely, Transformer-XL and GPT-2. These architectures are trained fully on WikiText-103 and One Billion Word (LM1B) datasets, which
% . Full training requires $40$K and $100$K steps on WikiText-103 and LM1B, respectively, and 
consumes over $\mathbf{25000}$ GPU-hours on NVIDIA A100 and V100 nodes. 
We compare the ranking obtained using decoder parameter count proxy and the ground truth ranking after full training in Figure~\ref{fig:zero_proxy}. On WikiText-103, zero-cost ranking using the decoder parameter count obtains a Spearman's Rank Correlation (SRC) of $0.97$ with full training. SRC further increases to $0.99$ for the more complex LM1B benchmark on both backbones. This validates that the decoder parameter count is strongly correlated with final model performance, thereby providing a reliable training-free proxy for NAS.
% Throughout the paper, we use the terms decoder parameter count and decoder parameter count interchangeably.



==> LTS_Version2 2/3_methodology.tex <==
\vspace{-0.3cm}
\section{Lightweight Transformer Search}\label{sec:methodology}
\vspace{-0.2cm}
% Figure~\ref{fig:overview} demonstrates a high-level overview of \sys{}. 
We perform an evolutionary search over candidate architectures
to extract models that lie on the Pareto-frontier. In contrast to the vast majority of prior methods that deliver a single architecture from the search space, our search is performed over the entire Pareto, generating architectures with a wide range of latency, peak memory utilization, and perplexity with one round of search. This alleviates the need to repeat the NAS algorithm for each hardware performance constraint.
% which spans a wide range of memory, latency, and perplexity characteristics. 

To evaluate candidate models during the search, \sys{} uses a training-free proxy for the validation perplexity. 
% This proxy metric along with real latency measurements on the target hardware are fed to the evolutionary search engine to guide the sampled architectures towards the Pareto-frontier. 
By incorporating training-free evaluation metrics, \sys{}, for the first time, performs the entire search directly on the target (constrained) hardware. Therefore, we can use real measurements of hardware performance during the search.
Algorithm~\ref{alg:algorithm} outlines the iterative process
\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-0.3cm}
\setlength{\algomargin}{8pt}
\begin{algorithm}[H]
\small
\DontPrintSemicolon
\SetNoFillComment
\SetAlgoLined
\KwIn{Search space $\mathcal{D}$, $n_{iter}$}
\KwOut{Perplexity-latency-memory Pareto-frontier $\mathbb{F}$}
$\mathcal{L}, \mathcal{M}, \mathcal{P}, \mathbb{F} \gets \emptyset, \emptyset,\emptyset, \emptyset$\;
\While{$N \leq n_{iter}$}{
    $\mathbb{F}' \gets$ Subsample($\mathbb{F}$)\;
    $\mathbb{S}_N \gets EA(\mathbb{F}', \mathcal{D})$\;
    \tcp{hardware profiling}
    $\mathcal{L} \gets \mathcal{L} \bigcup$ 
    Latency($\mathbb{S}_N$)\;
    $\mathcal{M} \gets \mathcal{M} \bigcup$ 
    Memory($\mathbb{S}_N$)\;
    \tcp{estimate perplexity}
    $\mathcal{P} \gets \mathcal{P} \bigcup$ Proxy($\mathbb{S}_N$)\;
    \tcp{update the Pareto-frontier}
    $\mathbb{F} \gets $ LowerConvexHull($\mathcal{P}, \mathcal{L}, \mathcal{M}$)
}
\caption{\sys{}'s training-free NAS}
\label{alg:algorithm}
\end{algorithm}
\vspace{-0.3cm}
\end{wrapfigure}
performed in \sys{} \footnote{The Pareto-frontier search method in Algorithm \ref{alg:algorithm} is inspired by \citep{elsken2018lemonade} and \citep{petridish2019}. Other possibilities include variations proposed in \citep{guerrero2021bagofbaselines}, evaluation of which is orthogonal to our contributions in this work.} for finding candidate architectures in the search space ($\mathcal{D}$), that lie on the $3$-dimensional Pareto-frontier ($\mathbb{F}$) of perplexity versus latency and memory. At each iteration, a set of points ($\mathbb{F'}$) are subsampled from the current Pareto-frontier. A new batch of architectures ($\mathbb{S}_N$) are then sampled from $\mathbb{F'}$ using evolutionary algorithms ($EA(.)$). The new samples are evaluated in terms of latency ($\mathcal{L}$), peak memory utilization ($\mathcal{M}$), and validation perplexity ($\mathcal{P}$). Latency and memory are measured directly on the target hardware while the perplexity is indirectly estimated using our accurate and training-free proxy methods. Finally, the Pareto-frontier is recalibrated 
% to incorporate the newly evaluated architectures. 
using the lower convex hull of all sampled architectures. In the context of multi-objective NAS, Pareto-frontier points are those where no single metric (e.g., perplexity, latency, and memory) can be improved without degrading at least one other metric~\cite{guerrero2021bagofbaselines}.
% The lower convex hull provides a conservative estimate of the Pareto-frontier. 
To satisfy application-specific needs, optional upper bounds can be placed on the latency and/or memory of sampled architectures during search.

% In what follows, we introduce the three components of \sys{} pipeline for NAS, namely, the search space, the validation perplexity proxy, and the evolutionary search. Throughout the paper, we will use the words `architecture' and `model' interchangeably.

% \vspace{-0.2cm}
% \subsection{Search Space}\label{sec:search_space}
\noindent\textbf{Search Space.}
Figure~\ref{fig:search_space} shows all elastic parameters in \sys{} search space, namely, number of layers (n\textsubscript{layer}), number of attention heads (n\textsubscript{head}), decoder output dimension (d\textsubscript{model}), inner dimension of the feed forward network (d\textsubscript{inner}), embedding dimension (d\textsubscript{embed}), and the division factor ($k$)  of adaptive embedding~\cite{baevski2018adaptive}. These architectural parameters are compatible with popularly used autoregressive
  \begin{wrapfigure}{r}{0.48\textwidth}\vspace{-0.3cm}
    \centering
    \vspace{-0.2cm}
    \includegraphics[width=0.37\columnwidth]{figures/search_space.png}
    \vspace{-0.2cm}
    \caption{Elastic parameters in \sys{} search space.}\label{fig:search_space}
\vspace{-0.2cm}
\end{wrapfigure}   
 Transformer backbones, e.g., GPT. For preliminaries on autoregressive Transformers, please see Appendix~\ref{sec:appdx_prelim}. We adopt a  heterogeneous search space where the backbone parameters are decided on a per-layer basis. This is in contrast to the homogeneous structure commonly used in Transformers~\cite{dai2019transformer,brown2020language}, which reuses the same configuration for all layers. Compared to homogeneous models, the flexibility associated with heterogeneous architectures enables them to obtain much better hardware performance under the same perplexity budget (see Section~\ref{sec:comparisons}). 

Heterogeneous search space was previously explored in~\cite{wang2020hat}. However, due to the underlying supernet structure, not all design parameters can change freely. As an example, the dimensionality of the \textit{Q, K, V} vectors inside the encoder and decoder layers is fixed to a large value of $512$ to accommodate inheritance from the supernet. 
Our search space, however, allows exploration 
of all internal dimensions without constraints. By not relying on the supernet structure, our search space easily encapsulates various Transformer backbones with different configurations of the input/output embedding layers and elastic internal dimensions. 

\sys{} searches over the following values for the architectural parameters in our backbones: n\textsubscript{layer}$\in \{2,\dots, 16|1\}$\footnote{We use the notation \{v\textsubscript{min},\dots, v\textsubscript{max}|step size\} to show the valid range of values.}, d\textsubscript{model}$\in \{128,\dots,1024|64\}$, d\textsubscript{inner}$\in \{256,\dots,4096|64\}$, and n\textsubscript{head}$\in \{2,4,8\}$. Additionally we explore adaptive input embedding~\cite{baevski2018adaptive} with d\textsubscript{embed}$\in \{128, 256, 512\}$ and factor $k\in\{1,2,4\}$. 
Once a d\textsubscript{model} is sampled, we adjust the lower bound of the above range for d\textsubscript{inner} to $2\times$d\textsubscript{model}. Encoding this heuristic inside the search ensures that the acquired models will not suffer from training collapse.
Our heterogeneous search space encapsulates more than $10^{54}$ different architectures. Such high dimensionality further validates the critical need for training-free NAS. 

% \mojan{The difference between the backbones are in Section~\ref{sec:setup}, should it be moved here?}


\vspace{-0.2cm}
\subsection{Training-free Architecture Ranking}\label{sec:proxies}
% In this section, we propose several training-free proxies for ranking Transformer architectures.
% during NAS. 
% \edit{We further provide extensive analysis and comparisons of the effectiveness and cost for each method on various benchmarks.}\mojan{might want to move this last part to the experiments}

\input{3_2_1_pruning}
\input{3_2_2_decoder_params}

\comment{
\vspace{-0.3cm}
\subsection{Evolutionary Search}
% \vspace{-0.1cm}
We use evolutionary algorithms to search over the candidate Transformer architectures. In contrast to the vast majority of prior methods that deliver a single architecture from the search space, our search is performed over the entire Pareto. As a result, \sys{} generates architectures with a wide range of latency, peak memory utilization, and perplexity characteristics with one round of search. This alleviates the need to repeat the NAS algorithm for each hardware performance constraint. At each iteration of the evolutionary search, we utilize our training-free proxy to rank the architectures in terms of their validation perplexity and measure the latency and peak memory utilization directly on the target hardware. We then estimate the Pareto-frontier of perplexity versus latency and memory using the lower convex hull of all sampled architectures. In the context of multi-objective NAS, Pareto-frontier points are those where no single metric (e.g., perplexity, latency, and memory) can be improved without degrading at least one other metric~\cite{guerrero2021bagofbaselines}.
% The lower convex hull provides a conservative estimate of the Pareto-frontier. 
The models on the Pareto-frontier are then used to sample new architectures using evolutionary operations, i.e., mutation and crossover. To satisfy application-specific needs, optional upper bounds can be placed on the latency and/or memory of sampled architectures during the search.
}

==> LTS_Version2 2/4_1_ranking_proxy.tex <==
\vspace{-0.2cm}
\subsection{How do training-free proxies perform compared to training-based methods?}\label{sec:exp_proxies}
\vspace{-0.1cm}
In this section, we benchmark several proxy methods for estimating the rank of candidate architectures. Specifically, we investigate three different ranking techniques, namely, partial training, low-cost methods, and number of decoder parameters.


\noindent $\blacktriangleright$ \textbf{Partial Training.} We first analyze the relationship between validation perplexity after a shortened training period versus that of full training for ranking candidate models. We stop the training after $\tau \in[1.25\%, 87.5\%]$ of the total training iterations needed for model convergence. Figure~\ref{fig:proxies} demonstrates the SRC and CR of partial training with various $\tau$s, evaluated on $100$ randomly selected models from the Transformer-XL backbone, trained on WikiText-103. The horizontal axis denotes the average time required for $\tau$ iterations of training across all sampled models.
% \mojan{these are homogeneous architectures}
Intuitively, a higher number of training iterations results in a more accurate estimate of the final perplexity. Nevertheless, the increased wall-clock time prohibits training during search and also imposes the need for GPUs. Interestingly, very few training iterations, i.e., $1.25\%$, provide a very good proxy for final performance with an SRC of $>0.9$ on the entire population. Our training-free proxy, i.e., decoder parameter count, also shows competitive SRC compared to partial training.

% This motivates us to investigate training-free methods as a performance proxy.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/partial_training.png}
    \vspace{-0.2cm}
    \caption{Comparison between partial training and our zero-cost proxy, i.e., decoder parameter count, in terms of ranking performance and timing overhead. Each subplot corresponds to a top$k\%$ of the randomly sampled models, based on their validation perplexity after full training.
    % \protect\footnotemark.}
    % CR is well-suited for evaluating the ranking on smaller subsets. As such, here we show CR for topk$\in\{10,30,50\}$. SRC is well-defined for evaluating the ranking over all sampled architectures. Therefore, we show SRC on topk$\in\{30,50,100\}$. }
}\label{fig:proxies}
\vspace{-0.5cm}
\end{figure}
% \footnotetext{We demonstrate CR and SRC for all topk values for the decoder parameter count proxy in Figure~\ref{fig:param_count}}

% \noindent $\blacktriangleright$ \textbf{Synaptic Flow.} The synaptic flow introduced in~\cite{tanaka2020pruning} assigns an importance score to \edit{CNN} weights that can be used to prune redundant parameters without need for training or utilizing data. Followup work~\cite{abdelfattah2020zero} has utilized the summation of synaptic flow score over all model weights to perform zero-shot NAS on CNNs. We adapt the formulation of synaptic flow to Transformer architectures. Specifically, since the embedding layer in Transformer architectures is equivalent to a look up table, we remove this layer in our analysis of the synaptic flow. 

% \mojan{mention that synaptic flow is a soft parameter counter}

% As shown in Figure~\ref{fig:proxies}, the synaptic flow proxy performs on par with partial training in terms of architecture ranking capabilities while incurring zero training cost. Therefore, the synaptic flow proxy improves the runtime for NAS by an average of \edit{$XXX$}. \edit{While synaptic flow does not require model training, it still requires one forward and backward pass over the architecture to compute the parameter scores, which can be time consuming on commodity hardware. Recent work~\cite{} has shown that the synaptic flow measure is equivalent to a soft parameter counter. As such, we propose to utilize the number of model parameters as a proxy for validation perplexity.} 

\noindent $\blacktriangleright$ \textbf{Low-cost Proxies.} We benchmark various low-cost methods introduced in Section~\ref{sec:proxies} on $200$ randomly sampled architectures from the Transformer-XL
backbone, trained on WikiText-103. 
% Our low-cost proxies include the proxies mentioned in Section \ref{sec:proxies}. 
Figure~\ref{fig:pruning} shows the SRC between low-cost proxies and the ground truth  ranking after full training.
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[h]
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=0.49\columnwidth]{figures/pruning.png}
    \vspace{-0.2cm}
    \caption{SRC between low-cost proxies and the ground truth ranking after full training of 200 randomly sampled Transformers. The decoder parameter count obtains the best SRC with zero cost.}\vspace{-0.3cm}
    \label{fig:pruning}
% \end{figure}
\end{wrapfigure}
% \footnote{\mojan{A similar analysis for the GPT-2 backbone is included in the supplementary material Figure~\ref{XXX}}}. 
We measure the cost of each proxy in terms of FLOPs. 
As seen, the evaluated low-cost proxies have a strong correlation with the ground truth ranking (even the lowest performing \relulogdet has $>0.8$ SRC), validating the effectiveness of training-free NAS on autoregressive Transformers. 
The lower performance of \relulogdet can be attributed to the much higher frequency of ReLU activations in CNNs, for which the method was originally developed, compared to Transformer-based architectures.  
% Nevertheless, the remaining low-cost proxies demonstrate a strong correlation with the ground truth ranking which validates the effectiveness of training-free NAS on autoregressive Transformers. 
Our analysis of randomly selected models with homogeneous structures also shows a strong correlation between the low-cost proxies and validation perplexity, with
decoder parameter count outperforming other proxies (see Appendix~\ref{sec:appdx_homogeneous}).

% The evaluated Transformers in Figure~\ref{fig:pruning} are randomly sampled from the heterogeneous search space introduced in Section~\ref{sec:search_space}. We provide a similar analysis of the proposed proxies on randomly selected Transformer models with homogeneous decoder blocks in the supplementary material, Appendix~\ref{sec:appdx_homogeneous}.

\noindent $\blacktriangleright$ \textbf{Parameter Count.} Figure~\ref{fig:param_proxy}a demonstrates the final validation perplexity versus the total number of model parameters for $200$ randomly sampled architectures from GPT-2 and Transformer-XL backbones.
This figure contains two important observations: (1)~the validation perplexity has a downward trend as the number of parameters increases, (2)~The discontinuity is caused by the dominance of embedding parameters when moving to the small Transformer regime. We highlight several example points in Figure~\ref{fig:param_proxy}a where the architectures are nearly identical but the adaptive input embedding factor $k$ is changed. Changing $k\in\{1,2,4\}$ (shown with different colors in Figure~\ref{fig:param_proxy}a) varies the total parameter count without much influence on the validation perplexity. 
% The randomly sampled architectures have adaptive input embedding~\cite{baevski2018adaptive} with factor $k\in\{1,2,4\}$, which generates a diverse range of embedding parameter counts without much influence on the validation perplexity. 

\begin{figure}[t]
    \centering
    % \begin{subfigure}[b]{0.28\textwidth}
    %  \centering
    %  \includegraphics[width=\textwidth]{figures/pareto_params_total.png}
    %  \caption{}
    % \label{fig:pareto_random}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.35\textwidth}
    %  \centering
    %  \includegraphics[width=\textwidth]{figures/common_ratio_spearman_topk_nparams_memformer_wt103.png}
    %  \caption{}
    %  \label{fig:param_count}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.35\textwidth}
    %  \centering
    %  \includegraphics[width=\textwidth]{figures/common_ratio_spearman_topk_nparams_gpt2_wt103.png}
    %  \caption{}
    %  \label{fig:param_count_gpt}
    %  \end{subfigure}
    \includegraphics[width=0.99\columnwidth]{figures/common_ratio_spearman_topk_nparams.png}
    %  \vspace{-0.2cm}
     \caption{(a) Validation perplexity after full training versus total parameters for $200$ randomly sampled architectures trained on WikiText-103. The clear downward trend suggests a strong correlation between parameter count and perplexity. (b), (c) Performance of parameter count proxies for ranking the randomly sampled architectures with Transformer-XL and GPT-2 backbones.
    % The decoder parameter count provides a very accurate ranking proxy with an SRC of $0.97$ over all samples. 
    % The total parameter count, however, has a low SRC and CR, due to the masking effect of large embedding parameter count.
    }\label{fig:param_proxy}
\vspace{-0.3cm}
\end{figure}

The above observations 
% and the empirical results noted by \citet{kaplan2020scaling} where decoder parameter count largely determines perplexity irrespective of Transformer architecture shape (see Fig 5 in \citep{kaplan2020scaling}), 
motivate us to evaluate two proxies, i.e., total number of parameters and decoder parameter count. 
% We benchmark the $300$ random architectures randomly sampled from Transformer-XL and GPT-2 backbones and study the parameter count proxies.
% over different model groups based on their validation perplexity.
Figures~\ref{fig:param_proxy}b and~\ref{fig:param_proxy}c demonstrate the CR and SRC metrics evaluated on the $200$ randomly sampled models divided into top$k\%$ bins based on their validation perplexity. As shown, the total number of parameters generally has a lower SRC with the validation perplexity, compared to decoder parameter count. This is due  to the masking effect of embedding parameters, particularly in the Transformer-XL backbone. The total number of decoder parameters, however, provides a highly accurate, zero-cost proxy with an SRC of $0.97$ with the perplexity over all models, after full training. We further show the high correlation between decoder parameter count and validation perplexity for Transformer architectures with homogeneous decoder blocks in the supplementary material, Appendix~\ref{sec:appdx_homogeneous}. While our main focus is on autoregressive, decoder-only, Transformers, we provide preliminary results on the ranking performance of parameter count proxies for encoder-only and encoder-decoder Transformers in Appendix~\ref{sec:appdx_domains}.

% \mojan{add raw numbers for spearman corr/common ratio inside a table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/common_ratio_spearman_topk_nparams.png}
%     \vspace{-0.3cm}
%     \caption{Performance of parameter count proxies for ranking $300$ randomly sampled architectures.
%     The decoder parameter count provides a very accurate ranking proxy with an SRC of $0.97$ over all samples. 
%     % The total parameter count, however, has a low SRC and CR, due to the masking effect of large embedding parameter count.
%     }\label{fig:param_count}
% \end{figure}

% Our zero-cost proxy outperforms all previously evaluated, higher cost, proxies as shown in Figures~\ref{fig:proxies} and~\ref{fig:pruning}. We thus propose using the decoder parameter count as the ranking proxy for the search.


% \begin{table}[h]
% \caption{}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lllccccccc@{}}
% \hline
% &
% & \multicolumn{3}{c}{Common Ratio} 
% & \multicolumn{4}{c}{Spearman's Corr} 
% \\ \cline{3-5} \cline{6-9}
% & \multicolumn{1}{r}{topk:}
% & 10     
% % & 30     
% & 50     
% & 10   
% & 30   
% & 50   
% & all   \\ \hline \hline
% \multicolumn{2}{l}{Snip}              
% & 0.70      
% % & 0.85      
% & 0.93      
% & 0.32    
% & 0.77    
% & 0.79    
% & 0.94  \\ \hline
% \multicolumn{2}{l}{GradNorm}
% & 0.55      
% & 0.78      
% & 0.93      
% & 0.30    
% & 0.79    
% & 0.77    
% & 0.90  \\ \hline
% \multicolumn{2}{l}{Fisher}            
% & 0.55      
% & 0.80      
% & 0.92      
% & 0.16    
% & 0.74    
% & 0.74    
% & 0.89  \\ \hline
% \multicolumn{2}{l}{JacobCov}          
% & 0.65      
% & 0.85      
% & 0.99      
% & 0.51    
% & 0.70    
% & \textbf{0.85}    
% & 0.97  \\ \hline
% \multicolumn{2}{l}{Grasp}             
% & 0.50      
% & 0.77      
% & 0.92      
% & 0.16    
% & 0.76    
% & 0.74    
% & 0.89  \\ \hline
% \multicolumn{2}{l}{ReLU-log-det}      
% & 0.55      
% & 0.75      
% & 0.73      
% & 0.64    
% & 0.55    
% & 0.76    
% & 0.80  \\ \hline
% \multicolumn{2}{l}{Synflow}           
% & 0.70      
% & 0.80      
% & 0.86      
% & 0.53    
% & 0.67    
% & 0.74    
% & 0.90  \\ \hline
% \multicolumn{2}{l}{Dec. Params} 
% & 0.60      
% & 0.85      
% & 0.84      
% & 0.71    
% & 0.66    
% & \textbf{0.85}    
% & \textbf{0.98}  \\ \hline
% \end{tabular}
% }
% \end{table}

\vspace{-0.2cm}
\subsection{How does variation in model topology affect decoder parameter count as a proxy?}\label{sec:topology}
\vspace{-0.2cm}

The low-cost proxies introduced in Section~\ref{sec:proxies}, rely on forward and backward passes through the network. As such, they automatically capture the topology of the underlying architecture via the dataflow. The decoder parameter count proxy, however, is topology-agnostic. In this section, we investigate the effect of topology on the performance of decoder parameter count proxy. Specifically, we seek to answer whether for a given decoder parameter count budget, the aspect ratio of the architecture, i.e., trading off the width versus the depth, can affect the final validation perplexity.  

We define the aspect ratio of the architecture as d\textsubscript{model} (=width), divided by n\textsubscript{layer} (=depth). This metric provides a sense of how skewed the topology is and has been used in prior works which study scaling laws for language models \citep{kaplan2020scaling}. For a given decoder parameter count budget, we generate several random architectures from the GPT-2 backbone with a wide range of the width-to-depth aspect ratios\footnote{We control the aspect ratio by changing the width, i.e., d\textsubscript{model} while keeping d\textsubscript{inner}=$2\times$d\textsubscript{model} and n\textsubscript{head}=$8$. The number of layers is then derived such that the total parameter count remains the same.}. The generated models span wide, shallow topologies (e.g., d\textsubscript{model}=$1256$, n\textsubscript{layer}=$2$) to narrow, deep topologies (e.g., d\textsubscript{model}=$112$, n\textsubscript{layer}=$100$). Figure~\ref{fig:scaling_exps_gpt_a} shows the validation perplexity of said architectures after full training on WikiText-103 versus their aspect ratio. The maximum deviation (from the median) of the validation perplexity is $<12.8\%$ for a given decoder parameter count, across a wide range of aspect ratios $\in[1,630]$. Our findings on the heterogeneous search space complement the empirical results by \cite{kaplan2020scaling} where decoder parameter count largely determines perplexity for homogeneous Transformer architectures, irrespective of shape (see Figure 5 in \citep{kaplan2020scaling}). 

% \begin{figure}[h]
% \vspace{-0.3cm}
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%      \centering
%     \includegraphics[width=\columnwidth]{figures/valid_ppl_scaling_exps.png}
%     \caption{}\label{fig:scaling_exps_a}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%      \centering
%      \includegraphics[width=\columnwidth]{figures/valid_ppl_latency_scaling_exps.png}
%     \caption{}\label{fig:scaling_exps_b}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%      \centering
%      \includegraphics[width=\columnwidth]{figures/valid_ppl_memory_scaling_exps.png}
%     \caption{}\label{fig:scaling_exps_c}
%     \end{subfigure}
%     % \includegraphics[width=\columnwidth]{figures/scaling_exps.png}
%     \vspace{-0.2cm}
%     \caption{Validation perplexity after full training versus (a) the width-to-depth aspect ratio, (b) latency, and (c) peak memory utilization. Models are randomly generated from the Transformer-XL backbone and trained on WikiText-103. For a given decoder parameter count, we observe low variation in perplexity across different models, regardless of their topology. The topology, however, significantly affects the latency and peak memory utilization for models with the same validation perplexity.}
%     \label{fig:scaling_exps}
%     % \vspace{-0.4cm}
% \end{figure}

% For deeper architectures (more than $40$ layers), we observe an increase in the validation perplexity, which results in a deviation from the pattern in Figure~\ref{fig:scaling_exps}a. This observation is associated with the inherent difficulty in training deeper architectures, which can be mitigated with proposed techniques in the literature~\cite{wang2022deepnet}. Nevertheless, such deep models have a high latency, which makes them unsuitable for lightweight inference. For the purposes of hardware-aware and efficient Transformer NAS, our search-space contains architectures with less than $16$ layers. In this scenario, the decoder parameter count proxy holds a very high correlation with validation perplexity, regardless of the architecture topology as shown in Figure~\ref{fig:scaling_exps}a. 

We observe stable training when scaling models from the GPT-2 backbone up to $100$ layers, with the perplexity increasing only when the aspect ratio nears $1$. Nevertheless, such deep models are not part of our search space as they have high latency and are unsuitable for lightweight inference. For the purposes of hardware-aware and efficient Transformer NAS, decoder parameter count proxy holds a very high correlation with validation perplexity, regardless of the architecture topology as shown in Figure~\ref{fig:scaling_exps_gpt_a}. 
We further validate the effect of topology on decoder parameter count proxy for the Transformer-XL backbone in Figure~\ref{fig:scaling_exps} of Appendix~\ref{sec:appdx_scaling}. Our results demonstrate less than $7\%$ deviation (from the median) in validation perplexity for different aspect ratios $\in[8,323]$. 
% Compared to GPT-2, models from the Transformer-XL backbone suffer from training collapse when layer size exceeds $40$. 
% and we only observe an increase in the perplexity when the aspect ratio reaches $1$. Our results validate that the decoder parameter count proxy over is applicable over a wide range of architectures.


Note that while models with the same parameter count have very similar validation perplexities, the topology in fact affects their hardware performance, i.e., latency (up to $2.8\times$) and peak memory utilization (up to $5.5\times$), as shown in Figures~\ref{fig:scaling_exps_gpt_b} and~\ref{fig:scaling_exps_gpt_c}. This motivates the need for incorporating hardware metrics in NAS to find the best topology. 

% \mojan{measure latency and memory for these models and show that they are different despite of having same number of parameters.}

\begin{figure*}[t]
\vspace{-0.2cm}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
     \centering
    \includegraphics[width=\columnwidth]{figures/valid_ppl_scaling_exps_gpt.png}
    \caption{}\label{fig:scaling_exps_gpt_a}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
     \centering
     \includegraphics[width=\columnwidth]{figures/valid_ppl_latency_scaling_exps_gpt.png}
    \caption{}\label{fig:scaling_exps_gpt_b}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
     \centering
     \includegraphics[width=\columnwidth]{figures/valid_ppl_memory_scaling_exps_gpt.png}
    \caption{}\label{fig:scaling_exps_gpt_c}
    \end{subfigure}
    % \includegraphics[width=\columnwidth]{figures/scaling_exps.png}
    \vspace{-0.2cm}
    \caption{Validation perplexity after full training versus the (a) width-to-depth aspect ratio, (b) latency, and (c) peak memory utilization. Models are randomly generated from the GPT-2 backbone and trained on WikiText-103. For a given decoder parameter count, we observe low variation in perplexity across different models, regardless of their topology. The topology, however, significantly affects the latency (up to $2.8\times$) and peak memory utilization (up to $5.5\times$) for models with the same perplexity.}
    \label{fig:scaling_exps_gpt}
    \vspace{-0.5cm}
\end{figure*}


==> LTS_Version2 2/4_2_zero-cost-NAS.tex <==
% \vspace{-0.2cm}
\section{How Good is the Decoder Parameters Proxy for Pareto-frontier Search?}\label{sec:nas}
In this Section, we validate whether the decoder parameter count proxy actually helps find Pareto-frontier models which are close to the ground truth Pareto front.
We first fully train all $1200$ architectures sampled from the Transformer-XL backbone during the evolutionary search (\ref{alg:algorithm}). Using the validation perplexity obtained after full training, we rank all sampled architectures and extract the ground truth Pareto-frontier of perplexity versus latency. We train the models on the WikiText-103 dataset and benchmark Intel Xeon E5-2690 CPU as our target hardware platform for latency measurement in this experiment. 

Figure~\ref{fig:nas} represents a scatter plot of the validation perplexity (after full training) versus latency for all sampled architectures during the search. The ground truth Pareto-frontier, by definition, is the lower convex hull of the dark navy dots, corresponding to models with the lowest validation perplexity for any given latency constraint. We mark the Pareto-frontier points found by the training-free proxy with orange color. As shown, the architectures that were selected as the Pareto-frontier by the proxy method are either on or very close to the ground truth Pareto-frontier. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/gt_pareto_latency_params.png}
%     \vspace{-0.3cm}
%     \caption{Perplexity versus latency pareto obtained from full training of $1200$ architectures sampled during NAS. Orange points present the pareto-frontier extracted using decoder parameter count proxy, which lies closely to the actual pareto-frontier. Decoder parameter count holds a SRC of $0.98$ with the ground truth perplexity after full training over all architectures.}
%     \label{fig:nas}
% \vspace{-0.4cm}
% \end{figure}

\begin{SCfigure}[50][h]
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/gt_pareto_latency_params.png}
    \vspace{-0.2cm}
    \caption{Perplexity versus latency Pareto obtained from full training of $1200$ architectures sampled during NAS on Transformer-XL backbone. Orange points are the Pareto-frontier extracted using decoder parameter count proxy, which lies close to the actual Pareto-frontier. Decoder parameter count holds an SRC of $0.98$ with the ground truth perplexity after full training.}
    \label{fig:nas}
\vspace{-0.2cm}
\end{SCfigure}

We define the mean average perplexity difference as a metric to evaluate the distance ($d_{avg}$) between the proxy and ground truth Pareto-frontier:
\addtolength{\abovedisplayskip}{-0.7ex}
\addtolength{\abovedisplayshortskip}{-0.7ex}
\addtolength{\belowdisplayskip}{-0.7ex}
\addtolength{\belowdisplayshortskip}{-0.7ex}
\begin{equation}
    d_{avg} = \frac{1}{N}\sum_{i=1}^N \frac{|p_i - p_{gt, i}|}{p_{gt, i}}  
\end{equation}
Here, $p_i$ denotes the $i$-th point on the proxy Pareto front and $p_{gt, i}$ is the closest point, in terms of latency, to $p_i$ on the ground truth Pareto front. The mean average perplexity difference for Figure~\ref{fig:nas} is $d_{avg}=0.6\%$. This small difference validates the effectiveness of our zero-cost proxy in correctly ranking the sampled architectures and estimating the true Pareto-frontier. In addition to the small distance between the prxoy-estimated Pareto-frontier and the ground truth, our zero-cost proxy holds a high SRC of $0.98$ over the entire Pareto, i.e., all $1200$ sampled architectures. 

\comment{
We provide the ranking performance for different evaluation techniques along with their cost in Table~\ref{tab:nas_cost}. As seen, our proposed evaluation proxy, i.e., decoder parameter count, provides the highest SRC with the ground truth ranking of the sampled architectures during NAS, while removing the extremely high overhead of training. 

\begin{SCtable}
% \vspace{-0.2cm}
\centering
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{lcccc}
\hline
& \begin{tabular}[c]{@{}c@{}}Train\\ Iter\end{tabular}
& \begin{tabular}[c]{@{}c@{}}GPU\\ Hours\end{tabular}
& \begin{tabular}[c]{@{}c@{}}$CO_2$e\\ (lbs)\end{tabular}
& SRC  
\\ \hline \hline
Full Training                     
& 40,000        
& 19,024    
& 5433                                                
& 1.0             
\\ \hline
\multirow{2}{*}{Partial Training} 
& 500           
& 231       
& 66                                                   
& 0.92            
\\ \cline{2-5}
& 5,000         
& 2690     
& 768                                                  
& 0.96            
\\ \hline
\# Decoder Params                 
& \textbf{0}             
& \textbf{0}         
& $\sim$\textbf{0}                                              
& \textbf{0.98}           
\\ \hline
\end{tabular}}
\caption{Comparison between training-based and the proposed training-free evaluation proxy on a real NAS benchmark. The SRC is computed on the entire population set of $1200$ models visited during the search. The training time is reported on the NVIDIA V100 GPU.}\label{tab:nas_cost}
\end{SCtable}
}

We further study the decoder parameter proxy in scenarios where the range of model sizes provided for search is limited. We categorize the total $1200$ sampled architectures into different bins based on the decoder parameters. Figure~\ref{fig:param_count_bins} demonstrates the SRC between the decoder parameter count proxy and the validation perplexity after full training for different model sizes. The proposed proxy provides a highly accurate ranking of candidate architectures even when exploring a small range of model sizes. 
% This, in turn, validates the usage and effectiveness of decoder parameter count in conducting NAS on efficient (small) Transformers and delivering low-latency and high performance models.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\columnwidth]{figures/spearman_bins_nparams.png}
%     \vspace{-0.2cm}
%     \caption{\edit{SRC between the decoder parameter count proxy and validation perplexity. Results are gathered on $1200$ models grouped into $5$ bins based on their decoder parameter count. Our proxy performs exceptionally well on the smaller spectrum of model sizes.}}
%     \label{fig:param_count_bins}
% \vspace{-0.5cm}
% \end{figure}
\begin{SCfigure}[50][h]
    \centering
    \includegraphics[width=0.35\columnwidth]{figures/spearman_bins_nparams.png}
    \vspace{-0.2cm}
    \caption{SRC between the decoder parameter count proxy and validation perplexity. Results are gathered on $1200$ models grouped into four bins based on their decoder parameter count. Our proxy performs well even when exploring within a small range of model sizes.}
    \label{fig:param_count_bins}
\vspace{-0.2cm}
\end{SCfigure}





==> LTS_Version2 2/4_3_Comparisons.tex <==
\vspace{-0.2cm}
\subsection{Pareto-frontier models for various hardware platforms}\label{sec:comparisons}

% The straightforward way to produce architectures of different latency/memory is varying the number of layers (layer-scaling)~\cite{vaswani2017attention,dai2019transformer}. 
% % Any sophisticated search technique must produce better Pareto-frontiers than layer-scaling to be worthwhile. 
% We therefore benchmark the Transformer-XL (base) and GPT-2 (small) models with homogeneous layers $\in [1, 16]$ as the baseline Pareto. We compare our NAS-generated architectures with layer-scaled backbone models and achieve better validation perplexity and/or lower latency and peak memory utilization. % We utilize various scalings of the Transformer-XL~\cite{dai2019Transformer} architectures as our baseline for NAS.
% % \edit{We set the Transformer-XL Base model proposed for WikiText-103 in~\cite{transformer_github} as the backbone of the baseline models.}
% % \mojan{Details of the baseline architectures can be found in Tables~\ref{tab:archs_transxl} and~\ref{tab:archs_gpt2} in the Appendix~\ref{sec:appdx_archs}.} 
% All baseline\footnote{The best reported result in the literature for GPT-2 or Transformer-XL might be different based on the specific training hyperparameters, which is orthogonal to our investigation.}
% % Optimizing the training hyperparameters for a given architecture is orthogonal to NAS.} 
% and NAS-generated models are trained using the same setup enclosed in Table~\ref{tab:training_hyperparams} of Appendix~\ref{sec:appdx_training}.

We run LTS on different target hardware and obtain a range of Pareto-optimal architectures with various latency/memory/perplexity characteristics. During search, we fix the adaptive input embedding factor to $k=4$ to search models that are lightweight while ensuring nearly on-par validation perplexity with non-adaptive input embedding.
% This choice reduces the memory footprint of the Transformer while ensuring nearly on-par validation perplexity with non-adaptive input embedding. As such, it is well aligned with our purpose to deliver Transformer architectures for constrained hardware platforms.
As the baseline Pareto, we benchmark the Transformer-XL (base) and GPT-2 (small) models with homogeneous layers $\in [1, 16]$. This is because 
the straightforward way to produce architectures of different latency/memory is varying the number of layers (layer-scaling)~\cite{vaswani2017attention,dai2019transformer}. We compare our NAS-generated architectures with layer-scaled backbones and achieve better validation perplexity and/or lower latency and peak memory utilization. All baseline\footnote{The best reported result in the literature for GPT-2 or Transformer-XL might be different based on the specific training hyperparameters, which is orthogonal to our investigation.}
and NAS-generated models are trained using the same setup enclosed in Table~\ref{tab:training_hyperparams} of Appendix~\ref{sec:appdx_training}. 

Figure~\ref{fig:nas_results} shows the Pareto-frontier architectures found by \sys{} versus the layer-scaled baseline. Here, all models are trained on the LM1B dataset (See Figure~\ref{fig:nas_results_wt103} in Appendix~\ref{sec:comp_wt103} for results on WikiText-103). Note that the Pareto-frontier search is performed in a $3$-dimensional space, an example of which is enclosed in Appendix~\ref{sec:appdx_3dpareto}, Figure~\ref{fig:3d_pareto}. For better visualization, in Figure~\ref{fig:nas_results} we plot $2$-dimensional slices of the Pareto-frontier with validation perplexity on the y-axis and one hardware performance metric (either latency or memory) on the x-axis.

As seen, in the low-latency regime, \sys{} consistently finds models that have significantly lower perplexity compared to naive scaling of the baseline Transformer-XL or GPT-2. On the Transformer-XL backbone, \sys{} finds architectures with an average of $19.8\%$ and $28.8\%$ lower latency and memory, while achieving similar perplexity compared to the baseline on ARM CPU. Specifically, the perplexity of the $16$-layer Transformer-XL base can be replicated on the ARM device with a lightweight model that is $1.6\times$ faster and utilizes $1.9\times$ less memory during execution. On the Corei7 CPU, the Pareto-frontier models found by \sys{} are on average $25.8\%$ faster and  consume $30.0\%$ less memory under the same validation perplexity constraint. In this setting, \sys{} finds a model that replicates the perplexity of the $16$-layer Transformer-XL base while achieving $1.7\times$ faster runtime and $1.9\times$ less peak memory utilization. The savings are even higher on the GPU device, where the NAS-generated models achieve the same perplexity as the baseline with average $30.5\%$ lower latency and $27.0\%$ less memory. Specifically, an \sys{} model with the same perplexity as the $16$-layer Transformer-XL base has  $2.5\times$ lower latency and consumes $2.0\times$ less peak memory on TITAN Xp.

On the GPT-2 backbone, NAS-generated models consume on average $11.8\%$ less memory while achieving the same validation perplexity and latency on an ARM CPU. The benefits are larger on Corei7 and TitanXP where the latency savings are $13.8\%$ and $11.9\%$, respectively. The peak memory utilization also decreases by $9.7\%$ and $12.9\%$, on average, compared to the baseline GPT-2s on Corei7 and TITAN Xp. Notably, NAS finds new architectures with the same perplexity as the $16$-layer GPT-2 with $1.3\times$, $1.5\times$ faster runtime and $1.2\times$ lower memory utilization on Corei7 and TITAN Xp.

\begin{comment}
{Transformer-XL:
arm: 6.3\% lower ppl for same latency, 12.1\% lower ppl for same memory. 19.8\% lower latency and 28.8\% less memory for same ppl.
corei7: 8\% lower ppl for same latency, 10.2\% lower ppl for same memory. 25.8\% lower latency and 30.0\% less memory for same ppl.
titanxp: 13.0\% lower ppl for same latency, 11.3\% lower ppl for same memory. 30.5\% lower latency and 27.0\% less memory for same ppl.

GPT-2:
arm: 2.2\% lower ppl for same latency, 3.4\% lower ppl for same memory less memory for same ppl. same latency and 11.9\% less memory for same ppl.
corei7: 4.4\% lower ppl for same latency, 2.3\% lower ppl for same memory. 13.8\% lower latency and  9.7\% less memory for same ppl.
titanxp: 5.9\% lower ppl for same latency, 5.1\% lower ppl for same memory. 11.9\% lower latency and 12.9\% less memory for same ppl.}
\end{comment}

Our heterogeneous search space allows us to find a better parameter distribution among decoder layers. Therefore, \sys{} delivers architectures with better performance in terms of perplexity, while reducing both latency and memory when compared to the homogeneous baselines.
We provide the architecture of all baseline and \sys{} models shown in Figure~\ref{fig:nas_results} in Tables~\ref{tab:archs_transxl}-\ref{tab:archs_gpt2} of Appendix~\ref{sec:appdx_archs}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/3d_paretos_lm1b.png}
    \vspace{-0.5cm}
    \caption{2D visualization of the perplexity versus latency and memory Pareto-frontier found by \sys{}, versus the scaled backbone models with varying number of layers, trained on the LM1B dataset. Architectural parameters for models shown here are detailed in Appendix~\ref{sec:appdx_archs}. }
    \label{fig:nas_results}
\vspace{-0.5cm}
\end{figure*}


\noindent $\blacktriangleright$ \textbf{Search Efficiency.}
The main component in \sys{} search time is the latency/peak memory utilization measurement for candidate architectures since evaluating the model perplexity is instant using the decoder parameter count.
Therefore, our search finishes in a few hours on commodity hardware, e.g., taking only $0.9$, $2.6$, and $17.2$ hours on a TITAN Xp GPU, Corei7 CPU, and an ARM core, respectively. To provide more context into the timing analysis, full training of even one $16$-layer Transformer-XL base model on LM1B using a machine with $8\times$ NVIDIA V100 GPUs takes $15.8$ hours. 
% Using decoder parameters as a proxy significantly reduces our search runtime, allowing it to finish in a few hours on commodity hardware. 
% Figure~\ref{fig:nas_time} shows \sys{}'s runtime when performing the search directly on our evaluated target devices. The main component in our search time is the latency/peak memory utilization measurement for candidate architectures since evaluating the model perplexity is instant using the decoder parameter count. To provide more context into the timing analysis, we also show the time required for training a $16$-layer Transformer-XL base model on a machine with $8\times$ NVIDIA V100 GPUs. decoder parameters as a proxy significantly reduces the search runtime, allowing it to finish in a few hours on commodity hardware, without need for high-end GPUs. 
Once the Pareto-frontier models are identified, the user can pick a model based on their desired hardware constraints and fully train it on the target dataset. \sys{} is an alternate paradigm to that of training large supernets; our search can run directly on the target device and GPUs are only needed for training the final chosen Pareto-frontier model after search.
% The cost of training this model is lower than the cost of training large supernets, particularly since our NAS is focused on low-latency and memory-efficient Transformers. 
% \sys{} also avoids the many difficulties associated with training supernets.

% The main component in our search runtime is the latency measurement for candidate architectures since evaluating the model perplexity is nearly zero cost using the decoder parameter count. As such, our entire NAS is faster than the pre-processing phase of HAT where they benchmark thousands of architectures to build the latency simulator. 

In Table~\ref{tab:nas_cost} we study the ranking performance of partial training ($500$ steps) versus the decoder parameter count proxy for evaluating $1200$ architectures from the Transformer-XL backbone during \sys{} search. Astonishingly the decoder parameter count proxy gets higher SRC compared to partial training, while effectively removing training from the inner loop of search for NAS. 
% This proxy can hence be effectively used in the inner loop of search for NAS. 

%  \begin{minipage}{\textwidth}
%   \begin{minipage}[b]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/NAS_time.png}
%     \captionof{figure}{Top: Search runtime on target hardware using our zero-cost evaluation proxy. Bottom: Training time of one 16-layer Transformer-XL base on $8\times$ V100 nodes. Full training of just one Transformer on LM1B requires substantially more compute resources compared to our search. 
%     % which searches thousands of architectures on the target hardware.
%     } \label{fig:nas_time}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\textwidth}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lcccc}
%     \hline
%     & \begin{tabular}[c]{@{}c@{}}Train\\ Iter\end{tabular}
%     & \begin{tabular}[c]{@{}c@{}}GPU\\ Hours\end{tabular}
%     & \begin{tabular}[c]{@{}c@{}}$CO_2$e\\ (lbs)\end{tabular}
%     & SRC \\ \hline \hline
%     Full Training                     
%     & 40,000        
%     & 19,024    
%     & 5433                                                
%     & 1.0 \\ \hline
%     \multirow{2}{*}{Partial Training} 
%     & 500           
%     & 231       
%     & 66
%     & 0.92 \\ \cline{2-5}
%     & 5,000         
%     & 2690     
%     & 768
%     & 0.96 \\ \hline
%     \# Decoder Params                 
%     & \textbf{0}             
%     & \textbf{0}         
%     & $\sim$\textbf{0}
%     & \textbf{0.98} \\ \hline
% \end{tabular}}
%       \captionof{table}{Comparison between training-based and the proposed training-free evaluation proxy on a real NAS benchmark. The SRC is computed on the entire population set of $1200$ models visited during the search. The training time is reported on the Nvidia V100 GPU.}\label{tab:nas_cost}
%     \end{minipage}
%   \end{minipage}

\begin{SCtable}[50][h]
\vspace{-0.3cm}
\centering
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{lcccc}
\hline
& \begin{tabular}[c]{@{}c@{}}Train\\ Iter\end{tabular}
& \begin{tabular}[c]{@{}c@{}}GPU\\ Hours\end{tabular}
& \begin{tabular}[c]{@{}c@{}}$CO_2$e\\ (lbs)\end{tabular}
& SRC  
\\ \hline \hline
Full Training                     
& 40,000        
& 19,024    
& 5433                                                
& 1.0             
\\ \hline
\multirow{2}{*}{Partial Training} 
& 500           
& 231       
& 66                                                   
& 0.92            
\\ \cline{2-5}
& 5,000         
& 2690     
& 768                                                  
& 0.96            
\\ \hline
\# Decoder Params                 
& \textbf{0}             
& \textbf{0}         
& $\sim$\textbf{0}                                              
& \textbf{0.98}           
\\ \hline
\end{tabular}}
\caption{Ranking abilities of full and partial training versus our proxy for $1200$ models sampled during \sys{} search. Training time is reported for WikiText-103 and NVIDIA V100 GPU. Decoder parameter count proxy obtains an SRC of $0.98$ using zero compute.}\label{tab:nas_cost}
\vspace{-0.5cm}
\end{SCtable}
% \vspace{-0.5cm}

% \begin{SCfigure}[50][h]
%      \centering
%     %  \vspace{-0.2cm}
%      \includegraphics[width=0.55\columnwidth]{figures/NAS_time.png}
%     %  \vspace{-0.7cm}
%      \caption{Top: NAS runtime on target hardware using our zero-cost evaluation proxy. Bottom: Training time of one 16-layer Transformer-XL base on $8\times$ V100 nodes. Full training of just one Transformer on LM1B requires substantially more compute resources compared to \sys, which searches thousands of architectures directly on the target hardware.}
%     %  \caption{Timing analysis of \sys{} running on various target hardware, in comparison with the training time of the Transformer-XL architecture on $8\times$ V100 nodes.}
%      \label{fig:nas_time}
% \vspace{-0.3cm}
%  \end{SCfigure}


==> LTS_Version2 2/4_4_opt.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/0shot-scatter1.png}
%     \caption{\sys{} Pareto-frontier models (dots) achieve a higher zero-shot accuracy with lower latency compared to the hand-designed OPT-$350$M model (triangle). Latency is measured on an A6000 NVIDIA GPU.
%     % Results on additional tasks are provided in Appendix~\ref{sec:appdx_opt}, Figure~\ref{fig:appdx_opt_0shot}. 
%     Architectural parameters for all models shown here are detailed in Appendix~\ref{sec:appdx_archs}. \mojan{possibly replace this figure with the avg acc one}}
%     \label{fig:opt_0shot_1}
%     \vspace{-0.5cm}
% \end{figure*}
\begin{SCfigure}[50][t]
    \centering
    \includegraphics[width=0.55\columnwidth]{figures/avg_acc_scatter.png}
    \caption{Average zero and one-shot accuracy obtained by \sys{} models (dots) and the baseline OPT-$350$M (triangle) across $14$ NLP tasks. Latency is measured on an A6000 NVIDIA GPU.
    Architectural parameters for all models shown here are detailed in Appendix~\ref{sec:appdx_archs}.}
    \label{fig:avg_acc_opt}
\vspace{-0.5cm}
\end{SCfigure}


\vspace{-0.2cm}
\subsection{Zero and one-shot performance comparison of \sys{} models with OPT}\label{sec:opt}

 \citet{zhang2022opt} open-source a set of pre-trained decoder-only language models, called OPT, which can be used for zero or few-shot inference on various NLP tasks. Below, we compare the performance of \sys{} Pareto-frontier models with the hand-designed OPT architecture in zero and one-shot settings. 
 
We use \sys{} to search for language models with a GPT-2 backbone which have $300$M to $500$M total parameters to compare with the $350$M parameter OPT. Our search space is detailed in Appendix~\ref{sec:appdx_opt}. The search is conducted with latency as the target hardware metric and decoder parameter count as a proxy for perplexity. Once the search concludes, We train $20$ models from the Pareto-frontier along with OPT-$350$M on $28$B tokens from the Pile~\cite{gao2020pile}. The pretrained models are then evaluated on $14$ downstream NLP tasks, namely, HellaSwag~\cite{zellers2019hellaswag}, PIQA~\cite{bisk2020piqa}, ARC (easy and challenge)~\cite{clark2018think}, OpenBookQA~\cite{mihaylov2018can}, WinoGrande~\cite{sakaguchi2021winogrande}, and SuperGLUE~\cite{wang2019superglue} benchmarks BoolQ, CB, COPA, WIC, WSC, MultiRC, RTE, and ReCoRD. The training hyperparameters and the evaluation setup are outlined in Appendix~\ref{sec:appdx_training}.
 Figure~\ref{fig:avg_acc_opt} shows the overall average accuracy obtained across all $14$ tasks versus the inference latency for \sys{} models and the baseline OPT. As shown, NAS-generated models achieve a higher average accuracy with lower latency compared to the hand-designed OPT-$350$M model. We provide a per-task breakdown of zero and one-shot accuracy in Appendix~\ref{sec:appdx_opt}, Figure~\ref{fig:appdx_opt}.
 
\noindent $\blacktriangleright$ \textbf{Zero-shot Performance.} Figure~\ref{fig:appdx_opt_0shot} demonstrates the zero-shot accuracy obtained by \sys{} and OPT-$350$M on the benchmarked tasks. 
% The zero-shot evaluation on remaining tasks along with few-shot evaluations are enclosed in Appendix~\ref{sec:appdx_opt}. 
Compared to the OPT-$350$M architecture, \sys{} finds models that achieve higher accuracy and lower latency in the zero-shot setting on all evaluated downstream tasks. 
% As shown in Figure~\ref{fig:opt_0shot_1}, the maximum achievable accuracy of our NAS-generated models is $0.8-7.0\%$ higher than OPT-$350$M with an average speedup of $1.2\times$. If latency is prioritized, \sys{} provides models which are, on average, $1.6\times$ faster and $0.3-4.6\%$ more accurate than OPT-$350$M.
Specifically, the maximum achievable accuracy of our NAS-generated models is $0.2-8.6\%$ higher than OPT-$350$M with an average speedup of $1.2\times$. If latency is prioritized, \sys{} delivers models which are, on average, $1.5\times$ faster and up to $4.6\%$ more accurate than OPT-$350$M . 

\noindent $\blacktriangleright$ \textbf{One-shot Performance.}
Similar trends can be observed for one-shot evaluation as shown for different tasks in Figure~\ref{fig:appdx_opt_1shot}. \sys{} Pareto-frontier models improve the per-task accuracy of OPT-$350$M on $12$ out of $14$ tasks by $0.1-8.0\%$, while achieving an average speedup of $1.2\times$. On the same tasks, \sys{} Pareto-frontier includes models that enjoy up to $1.6\times$ speedup over OPT-$350$M with an average $1.5\%$ higher accuracy. On the RTE task, the best \sys{} model has $0.4\%$ lower accuracy but $1.6\times$ faster runtime. On the WSC task, the best performing \sys{} model obtains a similar one-shot accuracy as OPT-$350$M, but with $1.5\times$ faster runtime. 
\comment{
In the $32$-shot setting (\mojan{Figure~\ref{fig:opt_32shot}} in Appendix~\ref{sec:appdx_opt}), \sys{} models outperform OPT-$350$M on $11$ out of $14$ tasks, delivering accuracy improvements as high as $17.9\%$ for an average $1.2\times$ lower latency. The latency savings can further be pushed up to $1.6\times$ for a lower average accuracy improvement of $4.0\%$ across different tasks.
}


% \mojan{Double check BoolQ and RTE performance in the 1-shot setting} 

% \mojan{Record, piqa, and arch-easy are not included in 32-shot numbers because of worse performance} 





==> LTS_Version2 2/4_experiments.tex <==
\vspace{-0.3cm}
\section{Experiments}\label{sec:experiments}
\vspace{-0.1cm}
We conduct experiments to seek answers to the following critical questions:

\noindent\circled{1} How well can training-free proxies perform compared to training-based methods for estimating the performance of Transformer models?

\noindent\circled{2} How does model topology affect the performance of the proposed decoder parameter proxy?

\noindent\circled{3} Can our training-free decoder parameter count proxy be integrated inside a search algorithm to estimate the Pareto-frontier? How accurate is such an estimation of the Pareto?

\noindent\circled{4} Which models are on the Pareto-frontier of perplexity, latency, and memory for different hardware?

\noindent\circled{5} How well do \sys{} models perform in zero and one-shot settings compared to hand-designed variants when evaluated on downstream tasks?

We empirically answer questions \circled{1}, \circled{2}, \circled{4}, and \circled{5} in Sections~\ref{sec:exp_proxies}, \ref{sec:topology}, \ref{sec:comparisons}, and~\ref{sec:opt} respectively. We further address question \circled{3} in Appendix~\ref{sec:nas} where we show the Pareto-frontier models extracted by the decoder parameter count proxy are very close to the ground truth Pareto-frontier with an average of $0.6\%$ perplexity difference. Additionally, we show the efficacy of the decoder parameter count proxy when performing search on different ranges of model sizes in Appendix~\ref{sec:nas}, Figure~\ref{fig:param_count_bins}.

\vspace{-0.2cm}
\subsection{Experimental Setup}\label{sec:setup}
Please refer to Appendix~\ref{sec:appdx_training} for information about the benchmarked datasets, along with details of our training and evaluation setup, hyperparameter optimization, and evolutionary search algorithm.

\noindent\textbf{Backbones.} We apply our search on two widely used autoregressive Transformer backbones, namely, Transformer-XL~\cite{dai2019transformer} and GPT-2~\cite{radford2019language} that are trained from scratch with varying architectural hyperparameters. The internal structure of these backbones are quite similar, containing decoder blocks with attention and feed-forward layers. The difference between the backbones lies mainly in their dataflow structure; the Transformer-XL backbone adopts a recurrence methodology over past states coupled with relative positional encoding which enables modeling longer term dependencies. 
% \mojan{This can be moved to Section~\ref{sec:search_space}?}

\comment{
\noindent\textbf{Datasets.} 
We conduct experiments on two datasets, WikiText-103~\cite{merity2016pointer} and LM1B~\cite{chelba2013one}. The datasets are tokenized
using word-level and byte-pair encoding for models with Transformer-XL and GPT-2 backbones, respectively.
% , resulting in a total number of \edit{XXX} and \edit{XXX} training tokens for WikiText-103 and LM1B, respectively. 

\noindent\textbf{Training and Evaluation.}
We adopt the open-source code by~\cite{transformer_github} and~\cite{huggingface} to implement the Transformer-XL and GPT-2 backbones, respectively. 
% All benchmarked models are trained for $40$K and $100$K steps on the WikiText-103 and LM1B datasets, respectively. 
For each backbone and dataset, we use the same training setup for all models generated by NAS. We provide details of our training hyperparameters in Table~\ref{tab:training_hyperparams} of the supplementary material.
% Specifically, we follow the training hyperparameters, i.e., batch size, optimizer, learning rate values and scheduler, provided in ~\cite{transformer_github}'s open-source repository.
% \sys{} uses validation perplexity and inference latency as the two objectives for evaluating the candidate architectures. 
Validation perplexity is measured over a sequence length of $192$ and $32$ tokens for WikiText-103 and LM1B datasets, respectively. Inference latency and peak memory utilization are measured on the target hardware for the sequence length, averaged over $10$ measurements. We utilize PyTorch's native benchmarking interface for measuring the latency and memory utilization of candidate architectures.
% For our selected Pareto optimal architectures, we report the average latency over $100$ measurements after eliminating the top and bottom $5\%$ of the values. 
% We leverage \sys{} to find Transformer models on three platforms representing embedded and server-grade hardware: ARM Cortex-A57 CPU, Intel Core i7 CPU, and Nvidia TITAN Xp GPU.
}

\noindent \textbf{Performance Criteria.} To evaluate the ranking performance of various proxies, we first establish a ground truth ranking of candidate architectures by training them until full convergence. This ground truth ranking is then utilized to compute two performance criteria as follows:

\noindent$\blacktriangleright$ \underline{Common Ratio (CR):} We define CR as the percentage overlap between the ground truth ranking of architectures versus the ranking obtained from the proxy. CR quantifies the ability of the proxy ranking to identify the top$k\%$ architectures based on their validation perplexity after full training.

\noindent$\blacktriangleright$ \underline{Spearman's Rank Correlation (SRC):} We use this metric to measure the correlation between the proxy ranking and the ground truth. Ideally, the proxy ranking should have high correlation with the ground truth over the entire search space as well as high-performing candidate models.

% \begin{itemize}[label=$\blacktriangleright$]
%     \item Common Ratio (CR): We define CR as the percentage overlap between the ground truth ranking of architectures versus the ranking obtained from the proxy methods for the top-$k\%$ of architectures. CR quantifies the ability of the proxy ranking method to identify the top-$k\%$ architectures among all candidates.

%     \item Spearman's Rank Correlation (SRC): We utilize this metric to measure the correlation between the proxy ranking and the ground truth. Similar to the CR, we report the SRC over various top-$k\%$; ideally, the proxy ranking shall have high correlation with the ground truth over the entire search space as well as high-performing candidate models.

% \end{itemize}

\comment{
\noindent \textbf{Search Setup.}
% Our candidate architectures are sampled from the following architecture hyperparameters: n\textsubscript{layer}$\in [3, 8]$, d\textsubscript{model}$\in \{64, 128, 256, 512\}$, d\textsubscript{inner}$\in [512, 2048]$, and n\textsubscript{head}$\in \{2,4,8\}$.
% Additionally we explore adaptive input embedding~\cite{baevski2018adaptive} with d\textsubscript{embed}$\in \{128, 256, 512\}$ and factor $k\in\{1,2,4\}$. 
%  Our NAS is powered by evolutionary algorithms. 
Evolutionary search is performed for $30$ iterations with a population size of $100$; the parent population accounts for $20$ samples out of the total $100$; $40$ mutated samples are generated per iteration from a mutation probability of $0.3$; and $40$ samples are created using crossover.
}

\input{4_1_ranking_proxy}
% \input{4_2_zero-cost-NAS}
\input{4_3_Comparisons}
\input{4_4_opt}





==> LTS_Version2 2/5_conclusion.tex <==
% \vspace{-0.3cm}
\comment{
\section{Conclusion}\label{sec:conclusion}
% \vspace{-0.2cm}
We empirically establish a critical insight that there exists a strong correlation between the number of decoder parameters and final model performance for autoregressive Transformers.
Building upon this finding, we develop an efficient on-device search algorithm (LTS) that outputs models on the Pareto-frontier of perplexity versus various hardware metrics, e.g., latency and peak memory utilization. LTS utilizes the decoder parameter count as a training-free and zero-cost proxy for relative ranking of architectures during search. 
% Notably, the proposed training-free evaluation proxy eliminates the need for high-end compute resources to conduct NAS. Rather, 
Our search can be performed locally on the target (constrained) platform, where hardware performance metrics, e.g., latency, are directly measured. 
% Using our training-free proxy, we can extract the perplexity versus latency Pareto-frontier of Transformers in a record breaking time of $<3$ hours on a commodity Intel Core i7 CPU. 
We provide large-scale proof-of-concept experiments on the effectiveness of decoder parameter count as a ranking proxy using $2900+$ autoregressive Transformers of varying size, backbones, and two large language datasets.
}

\vspace{-0.3cm}
\section{Limitations and Future Work}\label{sec:conclusion}
\vspace{-0.1cm}
Decoder parameter count provides a simple yet accurate proxy for ranking autoregressive Transformers. This should serve as a strong baseline for future works on Transformer NAS. Our focus is mainly on autoregressive, decoder-only transformers. We therefore, study perplexity as the commonly used metric for language modeling tasks. Nevertheless, recent literature on scaling laws for Transformers suggest a similar correlation between parameter count and task metrics may exist for encoder only (BERT-style) Transformers or encoder-decoder models used in neural machine translation (NMT)~\cite{ghorbani2021scaling}. Additionally, recent findings~\cite{tay2021scale} show specific scaling laws exist between model size and downstream task metrics, e.g., GLUE~\cite{wang2018glue}. Inspired by these observations, we provide preliminary studies that suggest parameter count proxies may be applicable to Transformers in other domains. Detailed investigations of such zero-cost proxies for NAS on heterogeneous BERT-style or NMT models with new performance metrics is an important future avenue of research.

\vspace{-0.2cm}
\section{Acknowledgements}
Professor Farinaz Koushanfar's effort has been in parts supported by the NSF TILOS AI institute, award number CCF-2112665.
